ClusterGraph: a new tool for visualization and compression of multidimensional data

Understanding the global organization of complicated and high dimensional data is of primary interest for many branches of applied sciences. It is typically achieved by applying dimensionality reduction techniques mapping the considered data into lower dimensional space. This family of methods, while preserving local structures and features, often misses the global structure of the dataset. Clustering techniques are another class of methods operating on the data in the ambient space. They group together points that are similar according to a fixed similarity criteria, however unlike dimensionality reduction techniques, they do not provide information about the global organization of the data. Leveraging ideas from Topological Data Analysis, in this paper we provide an additional layer on the output of any clustering algorithm. Such data structure, ClusterGraph, provides information about the global layout of clusters, obtained from the considered clustering algorithm. Appropriate measures are provided to assess the quality and usefulness of the obtained representation. Subsequently the ClusterGraph, possibly with an appropriate structure--preserving simplification, can be visualized and used in synergy with state of the art exploratory data analysis techniques.

==> nmeth_img/line_1.tex <==
\definecolor{xdxdff}{rgb}{0.49019607843137253,0.49019607843137253,1}

\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]

\clip(-1.5,-0.5) rectangle (1.5,0.5);


\draw [fill=xdxdff] (-1,0) circle (2.5pt);
\draw [fill=xdxdff] (1,0) circle (2.5pt);
\draw [fill=xdxdff] (0,0) circle (2.5pt);

\end{tikzpicture}


==> nmeth_img/line_2.tex <==
\definecolor{xdxdff}{rgb}{0.49019607843137253,0.49019607843137253,1}


\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]

\clip(-1.5,-0.5) rectangle (1.5,0.5);

\draw [line width=2pt] (1,0)-- (-1,0);

\draw [fill=xdxdff] (-1,0) circle (2.5pt);
\draw [fill=xdxdff] (1,0) circle (2.5pt);
\draw [fill=xdxdff] (0,0) circle (2.5pt);

\end{tikzpicture}


==> nmeth_img/pipeline_CG.tex <==
\definecolor{tab_blue}{HTML}{1f77b4}
\definecolor{tab_orange}{HTML}{ff7f0e}
\definecolor{tab_green}{HTML}{2ca02c}
\definecolor{tab_red}{HTML}{d62728}
\definecolor{tab_purple}{HTML}{9467bd}
\definecolor{tab_brown}{HTML}{8c564b}
\definecolor{tab_pink}{HTML}{e377c2}
\definecolor{tab_gray}{HTML}{7f7f7f}
\definecolor{tab_olive}{HTML}{bcbd22}
\definecolor{tab_cyan}{HTML}{17becf}



\tikzstyle{startstop} = [rectangle, rounded corners,
minimum width=1cm,
minimum height=1cm,text width=2.5cm,
text centered,
draw=black,
fill=tab_green!30]

\tikzstyle{startstop2} = [rectangle, rounded corners,
minimum width=1cm,
minimum height=1cm,text width=3cm,
text centered,
draw=black,
fill=tab_green!30]

\tikzstyle{io} = [rectangle, rounded corners,
minimum width=1cm,
minimum height=1cm, text centered, text width=2.5cm,
draw=black,
fill=tab_cyan!30]

\tikzstyle{process} = [rectangle, rounded corners,
minimum width=1cm,
minimum height=1cm,
text centered, text width=2.5cm,
draw=black,
fill=tab_orange!30]

\tikzstyle{decision} = [rectangle, rounded corners,
minimum width=1cm,
minimum height=1cm,
text width=2.5cm,
text centered,
draw=black,
fill=tab_purple!30]

\tikzstyle{decision2} = [rectangle, rounded corners,
minimum width=1cm,
minimum height=1cm,
text width=3cm,
text centered,
draw=black,
fill=tab_purple!30]

\tikzstyle{arrow} = [thick,->,>=stealth]

\begin{tikzpicture}[node distance=2cm]

\node (data) [startstop, text width=1cm, fill=tab_green!30] {Data};
\node (cluster) [process, right of=data, xshift=1cm] {Clustering Algorithm};
\draw [arrow] (data) -- (cluster);

\node (fully) [process, right of=cluster, xshift=1.5cm] {Fully connected ClusterGraph};
\draw [arrow] (cluster) -- (fully);

\node (conn1) [decision,  right of=fully, xshift=0.5cm, yshift=2cm] {Connectivity pruning};
\draw [arrow] (fully) -- (conn1);

\node (connResult) [startstop2,  above of=conn1,  yshift=0.5] {Summary of distances between clusters};
\draw [arrow] (conn1) -- (connResult);

\node (knn) [io, right of=fully, xshift=0.5cm, yshift=-2cm] {K-nearest neighbors graph on data};
\draw [arrow] (fully) -- (knn);

\node (md) [io, below of=knn, yshift=-0.5cm] {Metric Distortion pruning};
\draw [arrow] (knn) -- (md);

\node (mdResult) [startstop,  left of=md,  xshift=-1cm] {Graph which respects the best the geometry of data};
\draw [arrow] (md) -- (mdResult);

\node (merge) [decision, left of=mdResult, xshift=-1.5cm ] {Merge of disconnected component};
\draw [arrow] (mdResult) -- (merge);

\node (conn2) [decision2, left of=merge, xshift=-1.5cm, yshift=2cm ] {Connectivity pruning restricted to the edges added during the merge};
\draw [arrow] (merge) -- (conn2);

\node (conn2Result) [startstop, below of=conn2, yshift=-1.5cm ] {Clear relationship between components};
\draw [arrow] (conn2) -- (conn2Result);


\end{tikzpicture}

==> nmeth_img/triangle_1.tex <==

\definecolor{xdxdff}{rgb}{0.49019607843137253,0.49019607843137253,1}

\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]

\clip(-1.5,-0.1) rectangle (1.5,2);

\draw [fill=xdxdff] (-1,0) circle (2.5pt);
\draw [fill=xdxdff] (1,0) circle (2.5pt);
\draw [fill=xdxdff] (0,1.7320508075688772) circle (2.5pt);

\end{tikzpicture}

